CoCoLoFa: A Dataset of News Comments with Common Logical Fallacies Written by LLM-Assisted Crowds

Detecting logical fallacies in texts can help users spot argument flaws, but automating this detection is not easy. Manually annotating fallacies in large-scale, real-world text data to create datasets for developing and validating detection models is costly. This paper introduces CoCoLoFa, the largest known logical fallacy dataset, containing 7,706 comments for 648 news articles, with each comment labeled for fallacy presence and type. We recruited 143 crowd workers to write comments embodying specific fallacy types (e.g., slippery slope) in response to news articles. Recognizing the complexity of this writing task, we built an LLM-powered assistant into the workers' interface to aid in drafting and refining their comments. Experts rated the writing quality and labeling validity of CoCoLoFa as high and reliable. BERT-based models fine-tuned using CoCoLoFa achieved the highest fallacy detection (F1=0.86) and classification (F1=0.87) performance on its test set, outperforming the state-of-the-art LLMs. Our work shows that combining crowdsourcing and LLMs enables us to more effectively construct datasets for complex linguistic phenomena that crowd workers find challenging to produce on their own.

==> figures/confusion_matrix_James_vs_Fallacy.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/James_vs_Fallacy.png}
    \caption{
    The confusion matrix between the expert 2 annotations and \dataset labels.
    % \kenneth{Can we use larger fonts and more clear colors? This figure is just kinda hard to read.}
    %\kenneth{This is from the sample we sent to UpWork workers. TODOs: (1) Verify the labels are correct. (2) Any other comments or suggestions?}
    }
    \label{fig:confusion_matrix_james_vs_label}
\end{figure}

==> figures/confusion_matrix_Robert_vs_Fallacy.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/Robert_vs_Fallacy.png}
    \caption{
    The confusion matrix between the expert 1 annotations and \dataset labels.
    % \kenneth{Can we use larger fonts and more clear colors? This figure is just kinda hard to read.}
    %\kenneth{This is from the sample we sent to UpWork workers. TODOs: (1) Verify the labels are correct. (2) Any other comments or suggestions?}
    }
    \label{fig:confusion_matrix_robert_vs_label}
\end{figure}

==> figures/confusion_matrix_reddit_James_vs_Fallacy.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/Reddit_James_vs_Fallacy.png}
    \caption{
    The confusion matrix between the expert 2 annotations and Reddit labels.
    % \kenneth{Can we use larger fonts and more clear colors? This figure is just kinda hard to read.}
    %\kenneth{This is from the sample we sent to UpWork workers. TODOs: (1) Verify the labels are correct. (2) Any other comments or suggestions?}
    }
    \label{fig:confusion_matrix_reddit_james_vs_label}
\end{figure}

==> figures/confusion_matrix_reddit_Robert_vs_Fallacy.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/Reddit_Robert_vs_Fallacy.png}
    \caption{
    The confusion matrix between the expert 1 annotations and Reddit labels.
    % \kenneth{Can we use larger fonts and more clear colors? This figure is just kinda hard to read.}
    %\kenneth{This is from the sample we sent to UpWork workers. TODOs: (1) Verify the labels are correct. (2) Any other comments or suggestions?}
    }
    \label{fig:confusion_matrix_reddit_robert_vs_label}
\end{figure}

==> figures/confusion_matrix_reddit_Robert_vs_James.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/Reddit_Robert_vs_James.png}
    \caption{
    The confusion matrix of the annotation between two experts on the Reddit dataset.
    % \kenneth{Can we use larger fonts and more clear colors? This figure is just kinda hard to read.}
    %\kenneth{This is from the sample we sent to UpWork workers. TODOs: (1) Verify the labels are correct. (2) Any other comments or suggestions?}
    }
    \label{fig:confusion_matrix_reddit_robert_vs_james}
\end{figure}

==> sections/4-2-dataset-diversity.tex <==
% \input{tables/crowdsorucing_statistics}

% Table~\ref{tb:crowdsorucing_statistics} reports the statistics of the crowdsourcing task. 


%A common concern with using LLMs to synthesize data is the diversity of the data~\citep{lahoti-etal-2023-improving}.\kenneth{TODOs: add 1 or 2 good citations.}\samuel{should we mention this? because the topics and thread structures did not related to LLMs}
%This subsection examines the dataset's diversity in topics and dialogue structure.








\kenneth{TODO: This whole subsection can go to Appendix.}



% \input{tables/fallacy_statistics}

\paragraph{\dataset covers diverse topics.}
Table~\ref{tb:topic_statistics} shows the proportions of each topic in \dataset. 
As each news article may have multiple topics, the summation of each column may exceed 100\%. 
The result indicates that most of the news we collected is related to \emph{international relations}, \emph{women rights}, \emph{police brutality}, \emph{COVID/health issue}, \emph{freedom of speech}, \emph{digital rights}, and \emph{East Asian politics}.
%Only a small amount of news is corresponded to \emph{drug issue} and \emph{U.S. politics}.

\paragraph{\dataset contains comment sections with diverse thread structures.}
%As we collected the entire discussion thread for each news article, the structure and other comments of a discussion thread can serve as auxiliary information for identifying informal logical fallacies.
To analyze the structure of discussion threads in \dataset, we categorized the structures into four types:
\begin{itemize}[nosep]
    \item \textbf{Flat:} Every comment directly responds to the news article.
    \item \textbf{Single Conversation:} Only one comment received one or more replies.
    \item \textbf{Multiple Conversations:} Several comments received replies, but none of these replies received their own responses (no second-layer responses).
    \item \textbf{Complex:} Any structure that does not fit into the above categories.
\end{itemize}
%\kenneth{I tried to make it more clear. Does it make sense?}\samuel{yes}
We calculated the diversity of structures using the evenness index
%We also calculated the diversity of structures with the evenness index 
$J$, proposed by \citet{PIELOU1966131}:
\begin{align}
    J=H/\log S
\end{align}
where 
\begin{align}
    H=-\sum_i p_i \log p_i
\end{align}
$H$ is the Shannon Diversity Index~\citep{Shannon_1948}, $S$ is the total number of unique structures, and $p_i$ is the proportion of a unique structure within its category. 
The value of $J$ ranges from 0 to 1, with higher values indicating greater evenness in structure diversity.
Table~\ref{tb:thread_structure} shows the statistics for each thread structure type in \dataset.
In total, \dataset had 134 unique thread structures, most of which were of Single Conversation.
The diversity of thread structures was high. 
%particularly as the complexity of the structure increases.

%Note that there may still be relationships or discussions among comments in threads that are considered flat. 
%Table~\ref{tb:thread_structure} shows the statistics of the thread structures in the \dataset dataset.

==> sections/4-3-dataset-compare.tex <==
Table~\ref{tb:dataset_comparison} shows the comparison with three existing logical fallacy datasets: 


\begin{itemize}[nosep]

    \item \textbf{\textsc{Logic}}~\cite{Jin_Lalwani_Vaidhya_Shen_Ding_Lyu_Sachan_Mihalcea_Schoelkopf_2022}: A dataset consisting of common logical fallacy examples collected from online educational materials.
    
    \item \textbf{\textsc{LogicClimate}}~\citep{Jin_Lalwani_Vaidhya_Shen_Ding_Lyu_Sachan_Mihalcea_Schoelkopf_2022}: A dataset consisting of logical-fallacious sentences extracted from climate change news articles.
    
    \item \textbf{Reddit}~\citep{Sahai_Balalau_Horincar_2021}: A dataset consisting of fallacious and non-fallacious comments crawled from Reddit.
    
\end{itemize}

Compared to existing datasets, \dataset offers distinct advantages. Firstly, it sources instances from a simulated social media platform, a departure from datasets like \textsc{Logic} and \textsc{LogicClimate}, resulting in a more authentic representation of online discussions. Secondly, it stands as the largest logical fallacy dataset, containing 5,772 instances spanning over 20 topics, ensuring comprehensive coverage for training and evaluation. Notably, unlike the Reddit dataset, which provides limited context with only the thread title and up to three dependent comments, \dataset includes the entire news article and its corresponding discussion thread, enriching the context for fallacy identification.



Moreover, each instance in \dataset averages 4.19 sentences and 70 tokens, surpassing comparable datasets in both length and depth of context. This richness of context is pivotal for ensuring clarity and enhancing the precision of fallacy identification based on argument content and reasoning. Conversely, other datasets often consist of single-sentence instances, leading to a heightened reliance on argument structure for fallacy determination. Regrettably, this reliance introduces a risk of unreliability and bias in fallacy identification, as underscored by the low annotated agreement value reported by \citet{Sahai_Balalau_Horincar_2021}.


% the highest among comparable datasets. 
% This ample context proves essential for clarity and facilitates accurate fallacy identification based on argument content and reasoning. 
% In contrast, other datasets often comprise single-sentence instances; determining fallacies in those datasets usually highly (and falsely) rely on the structure of arguments. Unfortunately, this would introduce unreliability and potential bias in identifying fallacies, as evidenced by the low annotated agreement value reported by \citet{Sahai_Balalau_Horincar_2021}.
% In contrast, \dataset instances, with a minimum of two sentences and over four on average, enable more dependable fallacy identification based on argument content and reasoning.

% This ample context proves essential for clarity and facilitates accurate fallacy identification, contrasting with datasets often comprising single-sentence instances. The reliance on argument structure in such instances can introduce bias and unreliability, as evidenced by low annotated agreement values. 

==> tables/attack_classification.tex <==
\begin{table}[]
\centering
\small
\begin{tabular}{@{}l@{\hskip4pt}l@{\hskip8pt}c@{\hskip4pt}c@{\hskip4pt}c@{\hskip6pt}c@{\hskip4pt}c@{\hskip4pt}c@{}}
\toprule
                          \multirow{2}{*}{\makecell[bl]{Trained\\ On}} & \multirow{2}{*}{\makecell[bl]{Model}} & \multicolumn{3}{c}{Reddit}     & \multicolumn{3}{c}{\dataset}  \\ \cmidrule(lr){3-5}\cmidrule(l){6-8} 
                     &                  & P        & R        & F        & P        & R        & F       \\ \midrule
\multirow{2}{*}{Reddit}   & BERT                  & $69_{-2}$  & $68_{-2}$  & $68_{-2}$  & $71_{-2}$ & $70_{-2}$  & $67_{-1}$ \\
                          & NLI                   & $46_{-24}$ & $57_{-15}$ & $65_{-5}$  & $44_{-27}$ & $59_{-17}$ & $69_{-3}$ \\ \midrule
\multirow{2}{*}{\makecell[l]{\textsc{CoCo-}\\\textsc{LoFa}}} & BERT                  & $55_{-5}$  & $44_{-9}$  & $53_{+1}$  & $86_{-1}$  & $76_{-9}$  & $81_{-6}$ \\
                          & NLI                   & $58_{+4}$  & $52_{-12}$ & $52_{-2}$  & $84_{-5}$  & $85_{-4}$  & $85_{-4}$ \\ \midrule
                          & GPT-4                 & $73_{-11}$ & $69_{-11}$ & $69_{-11}$ & $85_{-3}$  & $84_{-2}$  & $84_{-2}$\\ \bottomrule
\end{tabular}
\caption{The result of context attack on the classification attack. All models have smaller performance decrease on \dataset, indicating its greater resilience to context attacks compared to the Reddit dataset.}
\label{tb:attack_classification}
\end{table}

==> tables/attack_detection.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[]
\centering
\small
\begin{tabular}{l@{\hskip4pt}lcccccccc}
\toprule
                          &       & \textsc{Logic} & \textsc{LogicClimate} & \multicolumn{3}{c}{Reddit}    & \multicolumn{3}{c}{\dataset}   \\ \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-7} \cmidrule(l){8-10}
Trained On                     & Model & R & R & P       & R        & F        & P        & R        & F        \\ \midrule
\multirow{2}{*}{Reddit}   & BERT  & $53_{+2}$        & $86_{+3}$               & $64_{-2}$ & $75_{+6}$  & $69_{+1}$  & $70_{-1}$  & $92_{+1}$  & $79_{-1}$  \\
                          & NLI   & $63_{+4}$        & $84_{+12}$              & $60_{-6}$ & $74_{+6}$  & $66_{-1}$ & $70_{-1}$ & $96_{+3}$ & $81_{+1}$  \\ \midrule
\multirow{2}{*}{\dataset} & BERT  & $55_{+1}$        & $83_{+6}$               & $63_{-2}$ & $56_{+12}$ & $59_{+6}$  & $83_{-3}$  & $80_{+4}$  & $82_{+1}$  \\
                          & NLI   & $67_{+14}$       & $87_{+11}$              & $54_{-4}$ & $58_{+15}$  & $56_{+5}$  & $77_{-4}$  & $90_{+7}$  & $83_{+1}$  \\ \midrule
                          & GPT-4 & $53_{-27}$       & $9_{-21}$               & $66_{+4}$ & $35_{-22}$ & $46_{-14}$ & $88_{+0}$  & $25_{-12}$ & $39_{-13}$ \\ \bottomrule
\end{tabular}
\caption{The result of context attack on the fallacy detection task. We reported the models' performance after the input was attacked, and calculated the discrepancy between the attacked and original performances, denoted by a subscript. GPT-4 exhibited contrasting behavior compared to finetuned models, indicating differences in their inference strategies.
% \kenneth{Instead of ``+2'' can we try ``~(+2)''? Feel more straightforward.}\samuel{then the attack\_classification table may not have enough space}
}
\label{tb:attack_detection}
\end{table*}

==> tables/cross-data-comp-kenneth-table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[t]
\centering
\footnotesize
\begin{tabular}{@{}cccccccccccccccccc@{}}
\toprule
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Model\\ Trained\\ On\end{tabular}}} & \multirow{3}{*}{\textbf{Model}} & \multicolumn{8}{c}{\textbf{Model Tested On (Original Dataset)}} & \multicolumn{8}{c}{\textbf{Model Tested On (Dataset After Attacked)}} \\ \cmidrule(l){3-18} 
 &  & \multicolumn{3}{c}{\textbf{D1 (Ours)}} & \multicolumn{3}{c}{\textbf{D2}} & \textbf{D3} & \textbf{D4} & \multicolumn{3}{c}{\textbf{D1 (Ours)}} & \multicolumn{3}{c}{\textbf{D2}} & \textbf{D3} & \textbf{D4} \\ \cmidrule(l){3-18} 
 &  & \textbf{P} & \textbf{R} & \textbf{F} & \textbf{P} & \textbf{R} & \textbf{F} & \textbf{R} & \textbf{R} & \textbf{P} & \textbf{R} & \textbf{F} & \textbf{P} & \textbf{R} & \textbf{F} & \textbf{R} & \textbf{R} \\ \midrule
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}D1\\ (Ours)\end{tabular}}} & \textbf{M1} & .aa & .bb & .cc & .dd & .ee & .ff & .gg & .hh & .aax & .bbx & .ccx & .ddx & .eex & .ffx & .ggx & .hhx \\
 & \textbf{M2} & .ii & .jj & .kk & .ll & .mm & .nn & .oo & .pp & .iix & .jjx & .kkx & .llx & .mmx & .nnx & .oox & .ppx \\ \midrule
\multirow{2}{*}{\textbf{D2}} & \textbf{M1} & .qq & .rr & .ss & .tt & .uu & .vv & .ww & .xx & .qqx & .rrx & .ssx & .ttx & .uux & .vvx & .wwx & .xxx \\
 & \textbf{M2} & .yy & .zz & .AA & .BB & .CC & .DD & .FF & .GG & .yyx & .zzx & .AAx & .BBx & .CCx & .DDx & .FFx & .GGx \\ \midrule
\multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}GPT-4\\ (Zero-Shot)\end{tabular}}} & .HH & .II & .JJ & .KK & .LL & .MM & .NN & .OO & .HHx & .IIx & .JJx & .KKx & .LLx & .MMx & .NNx & .OOx \\ \bottomrule
\end{tabular}
\caption{TABLE KENNETH}
\end{table*}

==> tables/crowdsorucing_statistics.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{lc}
        \toprule
        \# all workers participated & 100\\
        Max \# comments written by one worker & 681\\
        Avg. \# comments written by one worker & 39.9\\
        \# comments which replied to others & 877\\
        \# comments which have been responded & 731\\
        \bottomrule
    \end{tabular}
    % \vspace{-0.5pc}
    \caption{Statistics of the crowdsourcing task.}
    % \vspace{-1.5pc}
    \label{tb:crowdsorucing_statistics}
\end{table}

==> tables/fallacy_statistics.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{lccc}
        \toprule
        Fallacy & Train & Dev & Test \\
        \midrule
        Appeal to authority & 9.1\% & 7.3\% & 9.6\%\\
        Appeal to majority & 10.1\% & 10.4\% & 8.4\%\\
        Appeal to nature & 10.1\% & 10.6\% & 8.9\%\\
        Appeal to tradition & 10.2\% & 7.2\% & 9.1\%\\
        Appeal to worse problems & 9.8\% & 10.6\% & 11.7\%\\
        False dilemma & 10.2\% & 10.7\% & 10.7\%\\
        Hasty generalization & 10.4\% & 9.5\% & 8.6\%\\
        Slippery slope & 9.8\% & 11.6\% & 10.0\%\\
        None & 20.3\% & 22.2\% & 22.9\%\\
        \bottomrule
    \end{tabular}
    % \vspace{-0.5pc}
    \caption{Proportions of different fallacies in each split.}
    % \vspace{-1.5pc}
    \label{tb:fallacy_statistics}
\end{table}

==> tables/kappa_reddit.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{@{}l@{}ccc@{}}
        \toprule
        Fallacy & \makecell[cb]{Expert 1\\vs. Label} & \makecell[cb]{Expert 2\\vs. Label} & \makecell[cb]{Between \\Experts}\\
        \midrule
        Appeal to authority & 0.66 & 0.48 & 0.36\\
        Appeal to majority & 0.76 & 0.51 & 0.48\\
        Appeal to nature & 0.71 & 0.54 & 0.62\\
        Appeal to tradition & 0.64 & 0.53 & 0.49\\
        Appeal to worse problems & 0.53 & 0.56 & 0.52\\
        False dilemma & 0.56 & 0.41 & 0.36\\
        Hasty generalization & 0.46 & 0.20 & -0.03\\
        Slippery slope & 0.54 & 0.61 & 0.49\\
        None & 0.18 & 0.11 & 0.14\\
        \midrule
        Average & 0.56 & 0.44 & 0.38\\
        \bottomrule
    \end{tabular}
    % \vspace{-0.5pc}
    \caption{Cohen's $\kappa$ agreement between experts and Reddit's labels, as well as the agreement between two experts. 
    % Experts only agreed with Reddit's labels at a fair level ($\kappa\in[0.2,0.4]$) across most fallacy types. 
    % \kenneth{Can we add one more row for ``Overall'' at the bottom?}\samuel{checked}\kenneth{Okay maybe we don't need the Overall row...}
    }
    % \vspace{-1.5pc}
    \label{tb:kappa_reddit}
\end{table}
